Embedded Safe Reactive Navigation for Multirotors Systems using Control Barrier Functions

Aiming to promote the wide adoption of safety filters for autonomous aerial robots, this paper presents a safe control architecture designed for seamless integration into widely used open-source autopilots. Departing from methods that require consistent localization and mapping, we formalize the obstacle avoidance problem as a composite control barrier function constructed only from the online onboard range measurements. The proposed framework acts as a safety filter, modifying the acceleration references derived by the nominal position/velocity control loops, and is integrated into the PX4 autopilot stack. Experimental studies using a small multirotor aerial robot demonstrate the effectiveness and performance of the solution within dynamic maneuvering and unknown environments.

==> related_work.tex <==
\section{Related Work}\label{sec:related_work}

\begin{itemize}
    \item \textcolor{red}{Related Work must clarify the work we build upon here.}
\end{itemize}

Due to the critical nature of safety in aerial vehicles, extensive
work has been done regarding the application of CBFs for
unmanned aerial vehicles (UAVs), and in particular for multicopters.
The contribution in~\cite{exp_cbf}
introduces exponential CBFs to enforce high-level safety constraints
on high-order systems. The authors of \cite{cbf_cascaded_control}
develop a safe quadrotor controller using exponential CBFs inside
a Quadratic Program (QP) to ensure position and velocity constraints
within a cascaded controller.
In \cite{3d_quadrotor_safe_control} the authors demonstrate
safe navigation of a quadrotor in a cluttered environment
by enforcing constraints on the thrust for obstacle avoidance.
In \cite{cbf_apf_comparison}, the authors show that CBFs outperform
artificial potential fields for obstacle avoidance in an experiment
on planar navigation with a quadrotor.
The authors of \cite{mc_cbf_backstepping} propose a backstepping approach to enforce
constraints on position, velocity and rates, without a cascaded control,
and tested in simulation. In a recent work \cite{cbf_cone}, the authors
develop a new CBF construction for obstacle avoidance by ensuring
that the drone's velocity remains outside a cone of vectors that
may lead to collision.
In \cite{softmax_cbf}, the authors propose to combine locally measured obstacle
constraints into a single local CBF, and demonstrate the applicability
of the proposed approach on a simulated quadrotor in a 2D
environment.
In \cite{cbf_teleop}, the authors introduce a safety filter combined with
visual-inertial SLAM and 3D occupancy maps for safe teleoperation of a
micro aerial vehicle modeled as a discrete time system.
The work in \cite{learning_cbf} proposes a full-stack perception-driven
feedback controller using two
jointly-trained neural networks that estimate a CBF and a Control Lyapunov Function (CLF)
directly on the observation space of a robot. A similar approach
was proposed by \cite{neural_cbf} and experimentally tested
for indoor and outdoor flights with a quadrotor.
In a recent work \cite{dyn_cbf_mpc}, the obstacles are modeled
as a set of ellipses whose trajectory is estimated over time from
LiDAR observations. Finally, the local trajectory planner leverages
a dynamic CBF-based MPC to handle collision avoidance.
